Deployment of an Online Feedback Optimization Controller for Reactive Power Flow Optimization in a Distribution Grid

Optimization is an essential part of power grid operation and lately, Online Optimization methods have gained traction. One such method is Online Feedback Optimization (OFO) which uses measurements from the grid as feedback to iteratively change the control inputs until they converge to the solution of the optimization problem. Such algorithms have been applied to many power system problems and experimentally validated in lab setups. This paper implements an OFO controller in a real distribution grid for 24/7 operation using off-the-shelf hardware and software. The proposed control strategy optimizes the reactive power flow at the substation while satisfying voltage constraints. As part of an existing coordination scheme between (sub)transmission grid operator (TSO) and distribution grid operator (DSO), this comes with a financial reward and simultaneously it virtually reinforces the grid by regulating the voltage on the feeder and therefore allowing higher levels of distributed generation/consumption. We present how a distribution grid is retrofitted such that we can use existing inverters, we analyze the controller's interaction with legacy infrastructure, and investigate its overall control behavior. Finally, we demonstrate the successful deployment of an OFO controller in an operational environment which corresponds to Technology Readiness Level (TRL) 7.

==> Figures/bar_plot_active_reactive_AEW.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
%
\begin{tikzpicture}

\begin{axis}[%
width=0.951\fwidth,
height=\fheight,
at={(0\fwidth,0\fheight)},
scale only axis,
bar shift auto,
xmin=-0.200,
xmax=32.200,
xlabel style={font=\color{white!15!black}},
xlabel={Days},
ymin=-4000.000,
ymax=5000.000,
ylabel style={font=\color{white!15!black}},
ylabel={Energy [kVArh or kWh]},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot[ybar, bar width=0.8, fill=mycolor1, draw=black, area legend] table[row sep=crcr] {%
1.000	3177.120\\
2.000	2484.350\\
3.000	1006.890\\
4.000	1348.410\\
5.000	1849.540\\
6.000	1174.650\\
7.000	3166.710\\
8.000	871.570\\
9.000	2967.290\\
10.000	3041.360\\
11.000	624.650\\
12.000	1953.730\\
13.000	2208.260\\
14.000	2552.710\\
15.000	516.600\\
16.000	2207.510\\
17.000	1112.290\\
18.000	2475.220\\
19.000	3612.050\\
20.000	3606.600\\
21.000	2683.450\\
22.000	1949.990\\
23.000	314.490\\
24.000	775.430\\
25.000	359.900\\
26.000	616.230\\
27.000	581.050\\
28.000	1276.630\\
29.000	1549.740\\
30.000	4184.690\\
31.000	4184.760\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
-0.200	0.000\\
32.200	0.000\\
};
\addlegendentry{active}

\addplot[ybar, bar width=0.8, fill=mycolor2, draw=black, area legend] table[row sep=crcr] {%
1.000	-2258.980\\
2.000	-1625.900\\
3.000	2.380\\
4.000	-148.000\\
5.000	-1087.190\\
6.000	-91.410\\
7.000	-2244.990\\
8.000	67.230\\
9.000	-2139.830\\
10.000	-2134.090\\
11.000	189.880\\
12.000	-1081.020\\
13.000	-1400.240\\
14.000	-1524.520\\
15.000	209.720\\
16.000	-1227.080\\
17.000	94.930\\
18.000	-1558.640\\
19.000	-2476.010\\
20.000	-2581.430\\
21.000	-1687.990\\
22.000	-1103.480\\
23.000	255.840\\
24.000	182.350\\
25.000	285.200\\
26.000	235.060\\
27.000	246.490\\
28.000	-430.680\\
29.000	-198.270\\
30.000	-3055.270\\
31.000	-3101.730\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
-0.200	0.000\\
32.200	0.000\\
};
\addlegendentry{reactive}

\end{axis}
\end{tikzpicture}%
